Effect of rotation on wake vortices in stratified flow

Stratified wakes past an isolated conical seamount are simulated at a Froude number of $Fr = 0.15$ and Rossby numbers of $Ro = 0.15$, 0.75, and $\infty$. The wakes exhibit a K{\' a}rm{\' a}n vortex street, unlike their unstratified, non-rotating counterpart. Vortex structures are studied in terms of large-scale global modes, as well as spatially localised vortex evolution, with a focus on rotation effects. The global modes are extracted by spectral proper orthogonal decomposition (SPOD). For all three studied $Ro$ ranging from mesoscale, submesoscale, and non-rotating cases, the frequency of the SPOD modes at different heights remains coupled as a global constant. However, the shape of the SPOD modes changes from slanted `tongues' at zero rotation ($Ro=\infty$) to tall hill-height columns at strong rotation ($Ro=0.15$). A novel method for vortex centre tracking shows that, in all three cases, the vortices at different heights advect uniformly at about $ 0.9U_{\infty}$ beyond the near wake, consistent with the lack of variability of the global modes. Under system rotation, cyclonic vortices (CVs) and anticyclonic vortices (AVs) present considerable asymmetry, especially at $Ro = 0.75$. The vorticity distribution as well as the stability of AVs are tracked downstream using statistics conditioned to the identified vortex centres. At $Ro=0.75$, intense AVs with relative vorticity up to $\omega_z/f_{\rm c}=-2.4$ are seen with small regions of instability but all AVs evolve towards a more stable state. Recent stability analysis that accounts for stratification and viscosity is found to improve on earlier criteria.

==> sections_final/app_hydro.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%  Moved to thesis 

% \section{Analysis of the non-hydrostatic pressure} \label{app2} 

% \jy{(write an intro/connection paragraph to this appendix in the main text.)} 

% In the numerical modelling of geophysical flows where the horizontal length scales are much greater than the vertical length scales, and where strong stratification and/or rotation permits only very large wavenumbers of vertical overturning motions, the flow is usually assumed to be hydrostatic in the vertical direction.  Since the vertical momentum equation is replaced by the hydrostatic pressure balance, the strict requirement for the vertical grid to resolve the stratification length scale $U/N$, which is very small at high stratification, is released. The pressure-velocity coupling is achieved by solving a 2D Poisson equation instead of 3D, which further reduces significantly the computational cost. 

% The application of hydrostatic assumption in geophysical flows were mostly justified via scaling and order of magnitude arguments, for the large scale flows. \cite{marshall1997hydrostatic} critiqued this assumption and suggested that non-hydrostatic simulations are needed in order to resolve both the large and small scales. Here we provide numerical examination of the role that the non-hydrostatic component of pressure plays, in our simulations of the hill wakes at $Fr=0.15$ and $Ro=0.15,0.75, \infty$, and suggest that non-hydrostatic simulation may still be needed to correctly capture some of large scale features, such as the VS frequencies and global modes. 

% % and in \cite{billant2001self}

% % show in the present Appendix that  an important role in the dynamics , and suggest that hydrodynamic simulations that solves all three momentum equations are still needed to study this type of problem. 

% \begin{figure}[pt]\captionsetup[subfloat]{farskip=-12pt,captionskip=1pt}
%   \subfloat[]{{\includegraphics[width=.475\linewidth]{./figs/Buinf_hy_nh_inst.pdf}}}% 
%   \subfloat[]{{\includegraphics[width=.475\linewidth]{./figs/Buinf_hy_nh_mean.pdf}}}% 
%   \\ 
%   \subfloat[]{{\includegraphics[width=.475\linewidth]{./figs/Bu25_hy_nh_inst.pdf}}}% 
%   \subfloat[]{{\includegraphics[width=.475\linewidth]{./figs/Bu25_hy_nh_mean.pdf}}}% 
%   \\ 
%   \subfloat[]{{\includegraphics[width=.475\linewidth]{./figs/Bu1_hy_nh_inst.pdf}}}% 
%   \subfloat[]{{\includegraphics[width=.475\linewidth]{./figs/Bu1_hy_nh_mean.pdf}}}% 
%   \\ 
%   \caption{Pressure gradients $\partial p^* /\partial z, \partial p_{\rm NH}/ \partial z, \partial p_{\rm HY}/ \partial z$ (a,c,e), and their time-averages (b,d,f). Cases BuInf (a,b), Bu25 (c,d), and Bu1 (e,f). All pressure gradients are normalised with the reference scale for density variation $\Delta \rho g= -\rho_0 N^2 h $. In each plot, the top, middle, and bottom row are $\partial p^* /\partial z$, $\partial p_{\rm NH}/ \partial z$, and $\partial p_{\rm HY}/ \partial z$, respectively. }
%   \label{fig:hy_nh} 
% \end{figure} 


% The pressure and density are decomposed into the ambient and dynamic components as in \eqref{rho_a}-\eqref{p_a},  
% % \begin{align}
% %   p(x,y,x,t) = p_a(z) + p^*(x,y,z,t) \label{p_a} \\
% %   \rho(x,y,z,t) = \rho_a(z) + \rho^*(x,y,z,t), \label{rho_a}
% % \end{align} 
% where the ambient density is balanced by the ambient pressure in the steady state. 
% % below moved to my notes (JL)
% % \begin{equation}
% %   \rho_a(z) = \rho_0 + \bar{\rho}(z) = \rho_0 - \int_{z_0}^z \frac{\rho_0}{g} N^2 \, {\rm d}z = \rho_0 [1-\frac{N^2}{g}(z-z_0)]
% % \end{equation} is balanced by the ambient pressure in the steady state:  \begin{equation} 
% %   \frac{\partial p_a}{\partial z} = - \rho_a g. \label{ambient}
% % \end{equation} The integration of Eq. \eqref{ambient} gives \begin{equation}
% %   p_a(z) = p_0 - \rho_0 g [ (z-z_0) - \frac{N^2}{2g}  (z-z_0)^2 ]
% % \end{equation} that will be subtracted from the instantaneous pressure to obtain the dynamic pressure as in Eq. \eqref{p_a}. The dynamic pressure and density are interpreted as the perturbations due to fluid motions. 
% The $z$-momentum equation for $w$ under the Boussinesq approximation reads \begin{equation}
%   \frac{Dw}{Dt} = - \frac{1}{\rho_0} \frac{\partial p^*}{\partial z} + (\nu+\nu_{\rm sgs}) \nabla^2 w + b,  \label{z-mom}
% \end{equation} where the buoyancy force is defined as $b = -\rho^*g/\rho_0$. Under the hydrostatic assumption, the acceleration and viscosity terms in Eq. \eqref{z-mom} are assumed to be zero, resulting in the balance  of the hydrostatic pressure (herein referred as $p_{\rm HY}$) with gravity \begin{equation}
%   \frac{\partial p_{\rm HY}}{\partial z} = - \rho^* g. \label{hy}
% \end{equation} The residual part of \eqref{z-mom}, \begin{equation}
%   \frac{\partial p_{\rm NH}}{\partial z} = -\rho_0 \frac{Dw}{Dt}  + \rho_0 (\nu+\nu_{\rm sgs}) \nabla^2 w, \label{nh}
% \end{equation} is defined as the balance of the non-hydrostatic pressure ($p_{\rm NH}$), with the acceleration and the viscous terms. Equations \eqref{hy}-\eqref{nh} constitute the decomposition of the dynamic pressure into hydrostatic and non-hydrostatic components \begin{eqnarray}
%   p^*(x,y,z,t) =  p_{\rm HY}(x,y,z,t) + p_{\rm NH}(x,y,z,t). 
% \end{eqnarray} In this Appendix the dynamic effects of $p_{\rm HY}$ and $p_{\rm NH}$ will be discussed in terms of their vertical gradients, which transport the vertical momentum. We note that $p_{\rm HY}$ computed from our hydrodynamic simulation won't equal the pressure field computed from hydrostatic simulations, since the entire pressure-velocity coupling system is modified there. 



% In practice, we obtain from the simulations the vertical gradient of the dynamic pressure $\partial p^*/\partial z$, compute $\partial p_{\rm HY}/\partial z$ from the dynamic density $\rho^*$ as in \eqref{hy}, and denote their difference as $\partial p_{\rm NH}/\partial z$. Figure \ref{fig:hy_nh} visualise both $\partial p_{\rm HY}/\partial z$ and $\partial p_{\rm NH}/\partial z$ at the vertical central plane at $y=0$. 

% In the sense of mean wake below the top of the hill, in figure \ref{fig:hy_nh} (b,d,f) it appears that the density variation $-\rho^* g$ is balanced out by vertical pressure gradient $\partial p^*/\partial z$, in the wake. The dynamic pressure gradient ($\partial p^*/\partial z$) and the hydrostatic pressure gradient ($\partial p_{\rm HY}/ \partial z$) fields agree reasonably well, with the difference in between ($\partial p_{\rm NH}/\partial z$) vanishingly small. However, above the top of the hill where the internal gravity waves dominates, the non-hydrostatic pressure gradient is non-negligible, and is consistent among all three cases, representing the steady lee waves. Also, in the instantaneous near wake ($x/D<2$) in figure \ref{fig:hy_nh} (a,c,e) where turbulent motion dominates and the VS is initiated, $\partial p_{\rm NH}/\partial z$ is nearly at the same order of magnitude as $\partial p_{\rm HY}/\partial z$. Hence, in the simulation of hill wakes with hydrostatic models \citep{dong2007island,perfect2018vortex,srinivasan2021high}, neglecting terms other than the pressure gradient and the buoyancy terms in the $z$-momentum equation could lead to considerable error, such as damping the vertical correlation near the onset of VS motions, as well as the amplitude of internal waves.  

% We note that the validity of hydrostatic assumption in the instantaneous intermediate wake ($x/D>2$) doesn't imply lack of motions in the vertical direction, but just the time required for the hydrostatic balance \eqref{hy} to establish is shorter than the time-scale of vertical motions. Indeed, the vertical transport is quite strong as indicated by the density perturbation field (same as $\partial p_{\rm HY}/\partial z$) in figure \ref{fig:hy_nh} (e), in case Bu1. The same reason explains its validity in the mean wake. 

% Overall, we report as a {\it posteriori} the magnitude of the non-hydrostatic pressure calculated from an LES database, and conclude that even though the hydrostatic pressure balances quite well the buoyancy force, hydrodynamic simulations are still required to resolve the near wake and associated dynamics. This Appendix is meant be a reference as to what extent the hydrostatic assumption is correct, and a note of caution before conduction of other oceanic flow simulations, since direct or large-eddy simulations has yet been widely available in ocean modelling.  

% \jy{Can you compute on the central vertical plane $y=0$ the spatial correlation of $p$? }

% Hydrodynamic is not suitable for the present cases but might still be acceptable in the cases of \cite{perfect2018vortex} with lower stratification. 

% Given the difference we are seeing compared to Perfect, hydro sims are still needed even if the pNH is small...  

